Decentralized Cross-Network Identity Management for Blockchain Interoperation

Interoperation for data sharing between permissioned blockchain networks relies on networks' abilities to independently authenticate requests and validate proofs accompanying the data; these typically contain digital signatures. This requires counterparty networks to know the identities and certification chains of each other's members, establishing a common trust basis rooted in identity. But permissioned networks are ad hoc consortia of existing organizations, whose network affiliations may not be well-known or well-established even though their individual identities are. In this paper, we describe an architecture and set of protocols for distributed identity management across permissioned blockchain networks to establish a trust basis for data sharing. Networks wishing to interoperate can associate with one or more distributed identity registries that maintain credentials on shared ledgers managed by groups of reputed identity providers. A network's participants possess self-sovereign decentralized identities (DIDs) on these registries and can obtain privacy-preserving verifiable membership credentials. During interoperation, networks can securely and dynamically discover each others' latest membership lists and members' credentials. We implement a solution based on Hyperledger Indy and Aries, and demonstrate its viability and usefulness by linking a trade finance network with a trade logistics network, both built on Hyperledger Fabric. We also analyze the extensibility, security, and trustworthiness of our system.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> tex/backup/3_solution.tex <==
\section{Solution}\label{sec:solution}


We now present a decentralized identity management solution to fulfill the requirements stated in Section~\ref{sec:decentralized_group_identity_management}, and whose development was guided by the following design principles:

% \subsection{Design Goals}
\begin{compactitem}
\item The solution should not be tied to, or only applicable for, a particular DLT.
\item Networks and their participants should be free to choose identity registries and providers (or use their existing ones).
\item Networks must retain their autonomy while gaining the ability to interoperate universally.
\item No change should be required in a network's regular operation, nor should it be burdened with onerous additional configurations.
\end{compactitem}



\begin{figure}
	\centering 
	\includegraphics[width=0.9\linewidth]{fig/architecture.pdf}
	\caption{Architecture to enable identity plane exchanges}
	\label{fig:architecture}
\end{figure}


\subsection{Building Blocks}
We rely on existing decentralized identity management concepts and tools to serve as building blocks for our solution.

\begin{compactitem}
\item \textbf{Decentralized Identifiers (DIDs)} is a W3C draft~\cite{did} for self-sovereign identity (SSI). A DID is a URI that resolves to a DID Document that contains information about its subject like aliases and pseudonymns. It can contain public keys to authenticate the subject's signature and service endpoints for communication with the subject to obtain verifiable credentials (see further below). We assume each network participant possesses a DID, decoupling its external identity from its network affiliation. 

\item \textbf{Verifiable Credentials (VC)} is W3C specification on cryptographic digital credentials based on DIDs, used to certify claims about their holders\cite{vc}, who can then prove their claims to third parties using \textbf{Verifiable Presentations (VP)}.

\item \textbf{Distributed Verifiable Data Registry (VDR)} is a data registry based on distributed ledger principles to support identity management. Hyperledger Indy \cite{indy} is one such blockchain-based platform that maintains DID records through consensus. (\textit{Note}: our design will accommodate centralized DID registries too but we recommend Indy-like networks for optimal levels of decentralization.)

\item \textbf{Identity and Credential Messaging} in a platform-neutral and interoperable protocol is required for peer-to-peer exchange of DID records, VCs, and VPs among issuers, subjects and verifiers. An example (though our design can accommodate any equivalent) is the \textit{DIDComm protocol} in \textit{Hyperledger Aries}~\cite{aries}, which facilitates such exchanges with support for encryption using keys and service endpoints stored in registry DID records.

\end{compactitem}

\begin{figure*}[t]
\centering
 \includegraphics[width=\textwidth]{fig/protocol2.pdf}
 \caption{Identity Exchange Protocol}
 \label{fig:protocol}
\end{figure*}

\subsection{Architecture}

Two sets of modules are required to realize an identity plane protocol (Figure~\ref{fig:architecture}) - (i) a set of networks separate from the interoperating networks, collectively called \textit{Distributed Identity Infrastructure}, in which identity and credential records are maintained, and (ii) a set of agents within an interoperating network, collectively called \textit{Network Identity Managers}, each acting on behalf of a participant, syncing and validating identities across network boundaries, and recording foreign identities on the local ledger. 

\subsubsection{\textbf{Distributed Identity Infrastructure}}
This is a \textit{cloud} of what we term \textbf{Interoperation Identity Networks (IINs)}, which collectively provide a common root of trust for networks to sync identities and certificates. Each IIN consists of a \textit{verifiable data registry} built on distributed ledger principles. A canonical IIN in our architecture is implemented as a Hyperledger Indy network, a public permissioned ledger allowing open queries but restricting writes to designated \textit{stewards} and \textit{trustees} (possessing \textit{trust anchor} roles). Indy maintains \textit{credential schemas}, \textit{credential definitions} (public keys for authentication), and revocation lists on its ledger through consensus among a pool of nodes~\cite{indy, aublin2013rbft}. In our scenario, an IIN built on Indy enables trustworthy validation of networks' and their participants' characteristics by maintaining DID records for network participants, and artifacts for supporting verifiable credential issuance and validation.

\textbf{Trust Anchors}: An \textit{IIN} does not have a centralized source of trust. Instead, a trust basis is collectively created by \textit{trust anchors} (stewards and trustees in Indy), entities that possess ledger write privileges and which can issue DIDs and verifiable credentials to users. In our scenario, trust anchors validate network members' real-world identity as well as their participation (membership) in interoperating networks. 
An IIN trust anchor can be one of two types:
\textit{\textbf{(a) Organization identity validators:}} These anchors are responsible for associating DIDs of network participants  with their real-world or legal identities. The open (W3) standard for a DID does not mandate such an association~\cite{did,didusecase}, and only creating a DID does not inherently tie it to a legal identity. Indy supports the registration of such identity associated DIDs (called \textit{verinyms} in Indy parlance) by trust anchors possessing \textit{steward} or \textit{trustee} roles~\cite{indy-transactions}. These anchors, or organization identity validators, are expected to already possess well-known real-world identities. A participating organization in a network can register a verinym using a \textit{NYM transaction}, with a record getting created in an IIN ledger after the IIN node pool achieves consensus. The existence of a verinym record for a network participant implies that its identity is attested by one or more trust anchors of that IIN.

\textit{\textbf{(b) Participant membership validators:}} Verification of a  \textit{verinym} only attests the real world identity of an organization, but does not validate its membership in any permissioned blockchain network. Enterprise blockchain networks formed by mutual agreement among its participants have no single central authority that can certify the network's structure or its members. Therefore, proving participation of an organization requires attestation by one or more reputed trust anchors,which we call \textit{participant membership validators}, which like the \textit{organization identity validators} are reputed in industry or well-known as consortia representatives. For example, either IBM or Walmart, both reputed entities, could act as validators for the membership of the IBM Food Trust \cite{ibmfoodtrust} network, in whose launch and governance they both played key parts.
These trust anchors issue verifiable credentials to participants attesting their network memberships and also revoke them when organizations leave networks.
An organization may hold multiple VCs attesting its memberships in multiple networks. In a cross-network data sharing session, it can construct VPs proving its membership in the network that is participating in the data sharing protocol without revealing its memberships in other networks, thus ensuring privacy \cite{vc}.

\textbf{IIN  Artifacts:} Artifacts maintained in an IIN's ledger are:

\begin{compactitem}
\item \textit{Verinyms} attesting the real-world identity of an organization (network participant).

\item \textit{Membership VC} - Attests the participation of an organization in a certain blockchain network. The VC contains the organization's DID, and the name/identity of a network it is a member of, as attributes (claims). This \textit{Membership VC schema} is recorded on the IIN ledger, and every organization's VC must adhere to it, though different VCs may use different encodings and cryptographic algorithms. Corresponding to the schema is a \textit{Membership VC Definition}, or a public key, which is also recorded on the ledger and used to validate membership claims (verifiable presentations) made by a holding organization.

\item \textit{Memberlist VC} - This consists of a name/identifier for a given network and a list of the network's participants' DIDs as schema attributes. Memberlist VCs are issued by participant membership validators, and are used by interoperating networks to fetch their counterparty networks' list of participants, after which each participant's membership VC can be fetched and validated. 

\item \textit{Revocation Registries} - When a blockchain network's member leaves, its \textit{Membership VC} indicating affiliation with the network must be revoked. We use cryptographic accumulators~\cite{accumulators} as revocation registries, allowing membership presence checks without revealing the entire list of members. Each \textit{Membership VC} issuer registers a separate revocation registry on the IIN ledger. This registry is updated when a VC is revoked, and is also looked up by entities validating a verifiable presentation made by a Membership VC holder.

\end{compactitem}

\subsubsection{\textbf{Network Identity Managers }}
These are components that run within the trust boundary of a permissioned network, one or more acting on behalf of each participating organization. A network identity manager is responsible for identity-syncing, i.e., (i) presenting its own identity and membership credentials to a foreign network, and (ii) correspondingly validating the membership credentials of a foreign network's members, and fetching and storing their certificates in the local ledger for data plane interoperation. We will henceforth refer to these managers as IIN Agents as they rely on IINs and their trust anchors for discovery and connections with foreign networks.

\textbf{IIN Agents:} An \textit{IIN Agent} is the identity managing component of a participant that creates its DID, registers it as verinym, and obtains Membership VCs from trust anchors in the IIN. It communicates with IIN Agents of foreign network's participants to present its own identity, as well as validate their identity and membership claims through VPs. 
More importantly, the \textit{IIN Agents} exchange their  blockchain specific identity and certificates as a self signed VPs that can be verified against their verinym. Once verified, they configure these certificates in their network's shared ledger through consensus.
This maps the decoupled SSI of the participants to their network specific identity, which ultimately makes proof verification possible in the data plane for interoperation. The inter IIN Agent exchanges can be implemented using the Aries DIDComm protocol \cite{aries} that enables confidential peer-to-peer communications.

\textbf{Interoperating Network Ledger Artifacts:} Each permissioned network must have a shared configuration detailing its policies on identity sharing, trust, and interoperation.
This configuration is expressed using the following ledger artifacts exposed through the \textit{configuration management system contract}~\cite{abebe2019enabling}:

\begin{compactitem}
\item \textit{Interoperation network list} - list of foreign networks to interoperate with.
\item \textit{Trust list} - which IINs to trust for identity and membership validation, as well as the trust anchors to use for specific interoperating networks.
\item \textit{Foreign network identities} - identities of participants (organizations/units) of foreign networks and their in-network credentials (typically certificate chains).
\end{compactitem}

\subsection{Identity Exchange Protocol}
\label{subsec:messageflow}
Figure \ref{fig:protocol} illustrates the steps in our canonical identity plane protocol to discover and sync identity and credentials across an example pair of networks (Network A and Network B) and a single IIN. Here, Org1 and Org2 in Network A are learning about the identity and membership of Org3 in Network B so both networks can interoperate for data-sharing. It is to be noted that by repeating the same steps, identity information of any of the other organizations in Network B can be discovered, fetched, validated and configured in Network A.

\textbf{\textit{(A) Configure DID and Membership VC:}} Org3 creates a DID, and  requests an organization identity validator to attest its identity and register it as a verinym. 
Once the verinym is registered in the IIN, Org3 has to get a Membership VC issued to it by suitable trust anchors. For that it requests one or more such membership validators who issue Membership VC with Org3 as the holder, and also updates the revocation registry to mark it as valid.
\textbf{\textit{(B) Validate DID \& Membership:}} Before starting the validation process, Org1 and Org2 need to know who the participants of Network B are. Org1 requests Memberlist VC from the membership validator, which returns a self signed VP. After the participants' DIDs of Network B are known, Org1 resolves Org3's DID Document from the Indy ledger.  This DID Document contains the service endpoint which is then used by Org1 to request Membership VP from Org3. Org1 then validates the VP received using the Membership VC schema, definition, and the revocation list, all fetched from the Indy ledger. 
\textbf{\textit{(C) Fetch Blockchain Identity Information:}} Org1 requests for blockchain identity artifacts (certificates), which are provided by Org3 in the form of a self signed VP that is validated against Org3's DID keys.
\textbf{\textit{(D) Update Identity in Ledger:}} Though Org1 now has verified the identities of Org3, there has to be some consensus among Network A's participants before this information is stored in the local ledger. Therefore, Org2 independently carries out steps (B) and (C) above and endorses Org1's transaction request to commit Org3's identity to the blockchain. Thus, no single party can unilaterally control the local representation of the identity of remote organizations.


==> tex/backup/4_implementation.tex <==
\section{Use Case for Hyperledger Fabric}\label{sec:implementation}

% Preamble
% Mention LC transfer
We demonstrate a proof-of-concept implementation of the protocol by augmenting the two-network use case in Abebe et al \cite{abebe2019enabling}. We started with the already developed scaled-down versions of the trade logistics network, TradeLens~\cite{tradelens}, and the trade finance network, We.Trade~\cite{wetrade}, namely \textit{Simplified TradeLens (STL)} and \textit{Simplified We.Trade (SWT)} respectively. Here, each network is a set of Docker containers 
% (run using \textit{docker-compose}) 
running Hyperledger Fabric peers, membership service providers (MSP), and an ordering service; application or client-layer components were also containerized. Further, each network was equipped with a relay and two system contracts: Configuration Management and Data Acceptance Chaincode (CMDAC) and Exposure Control Chaincode (ECC).

STL consists of a Seller and a Carrier organization, as illustrated in Figure~\ref{fig:trade-flow-implementation} each running one peer and one CA (serving as MSP). Consignments are created and dispatched in the workflow, with a bill of lading~\cite{billoflading} (B/L) recorded on ledger. SWT consists of a Seller and a Buyer organization, each with 2 peers and CAs, running a letter of credit~\cite{letterofcredit} (L/C) management workflow. SWT application clients include the same Seller that is a member of STL, a Buyer, and the Seller's and Buyer's banks. The interoperation steps are: (1) transfer of L/C from SWT to STL as a prerequisite for consignment creation and (2) transfer of B/L from STL to SWT in order to enforce payment obligation. 
% To the existing interoperation step, where the B/L is transferred from STL to SWT (Step 11) was added another (Step 6) where the L/C is transferred from SWT to STL as a prerequisite for consignment creation. The data plane query-response protocol remains the same as in Abebe et al.


\begin{figure}[t]
 \includegraphics[width=0.48\textwidth]{fig/trade_flow}
 \caption{Simplified Cross-Network Trade Use Case}
 \label{fig:trade-flow-implementation}
\end{figure}

% Fabric network 
\subsection{Fabric Network Organizations and Identity Providers}
We briefly describe how identity is managed within a Hyperledger Fabric network, which is a consortium of \textit{organizations} maintaining one or more \texttt{channels} (shared ledgers). Identity is independently managed within an organization by one or more \textit{membership service providers} (MSPs)~\cite{fabric-msp}, implemented as a set of Fabric CA Servers~\cite{fabric-ca-server} (CA: \textit{Certificate Authority}). Multiple root and intermediate CAs can exist within an organization, creating trust chains. Each peer or transaction-submitting client \textit{enrolls} with an MSP (one of the Fabric CA servers) in their organization to obtain a unique identity and X.509 certificates for transaction signing. Organizations are then linked together on a channel when a configuration block containing their respective MSPs' root and intermediate CA certificates is appended to that channel's blockchain.

Every transaction in a block must carry a set of peer signatures (according to an \textit{endorsement policy}) to be valid. Likewise, in our data-sharing interoperation protocol, any data shared with an external network can only be deemed valid if it carries a set of peer signatures that satisfies a \textit{verification policy}. But proof verification (i.e., signature validation) requires the destination network to possess the source network's organization list and their respective MSPs' certificates. It is here that IIN Agents play a key role, fetching certificates and creating identity records on the ledger using the CMDAC . Let us see how these agents are incorporated in a Fabric network.

%Hyperledger Fabric being a permissioned blockchain platform uses digital signatures for consensus, as well as to determine the permissions over resources that different participants have. Each participant might have multiple actors, - peers and applications. Therefore, each actor need their own set of identities and keys. All these identities are handled by Fabric's Membership Service Provider (MSP) , which is responsible for issuing  X.509 certificates. The MSP of an organization has a root certificate, from which all other certificates are derived for different actors. Thus the root certificate and the intermediate certificates form the basis of verifying endorsements in consensus process, and more importantly here, they are used for for validating proofs for interoperation in terms of  verifiable data transfer as described in Abebe et al \cite{abebe2019enabling}. The Fabric CA server is an embodiment of MSP (\textcolor{red}{ to be modified by Rama}). Generally there is one Fabric CA per organization that handles issuance of the identities.

%During interoperation, data arriving from a network is accompanied with proofs. For validation of these proofs, the X.509 root and intermediate certificates of the attesting organizations are required. These certificates are therefore configured in the CMDAC chaincode in the ledger, from which they are fetched by the proof validating chaincodes. Depending on the blockchain platform, these identities can be in some format other than X.509, with different cryptographic algorithms in use.
%Fabric peers are the components that can send transactions to the ledger, and therefore the peers have to execute the CMDAC chaincode to update identity information for interoperation that are being fetched and validated by the IIN Agent. We discuss next, how we implement IIN Agents for Fabric. 


\begin{figure}[t]
\centering
 \includegraphics[width=0.44\textwidth]{fig/implementation.jpg}
 \caption{IIN Components and Connections for Fabric}
 \label{fig:implementation}
\end{figure}

\subsection{IIN Agents within a Fabric Network}

% In our IIN architecture, each organization has an \textit{IIN Agent} which responsible for handling its identity information. This includes creating, and maintaining the blockchain independent identity - SSI, as well as querying the up-to-date blockchain specific identities for providing it to other interoperating organizations.
An IIN Agent represents an organization outside its network, and hence is designed to be an extension of that organization's MSP. 
% (Though an organization may employ multiple MSPs, a single one is typically used in production, and we will assume that to be the case here. If multiple MSPs are used, we can use a different Agent for each MSP, corresponding to an identifiable unit within the organization.) 
An organization typically uses a single MSP in production, but if multiple MSPs are used, representing organizational units, we can use a different Agents for each.
Logically, the Agent functionality ought to be performed by a Fabric CA Server.
% but there are different ways of implementing it. 
Rather than modifying the Fabric CA code, for implementation and deployment convenience, our IIN Agent is built as a decoupled service exposing an API for communication with IINs (Indy networks), IIN Agents of other local network organizations, and IIN Agents of foreign networks' organizations (see Figure~\ref{fig:implementation}). The IIN Agent also has client privileges and can submit transactions to the CMDAC. 
%In a Fabric network, the Fabric CA has the role of managing identities by issuing certificates and keys for the actors of the \textit{data plane}. Therefore, we have implemented the IIN Agent as its logical component (Figure \ref{fig:implementation}).
%Each IIN Agent has 4 interfaces, - (a) for managing SSI in  the Indy ledger - marked with blue arrows in Figure \ref{fig:implementation}, (b) for communicating with IIN Agent of other organizations and trust anchors - yellow arrows, (c) for fetching blockchain specific identity information - green arrow, and (d) to update foreign organizations' identities in CMDAC - grey arrows. 

An IIN Agent is composed of three modules. An \textit{Indy Agent} built using with \texttt{indy-sdk}\cite{indy-sdk} is used to connect to an IIN's Indy pool and query DID/credential information. An \textit{Aries Agent}, implemented using \texttt{ACA-Py}\cite{aca-py}, is used to communicate with IIN trust anchors for verinym, VC, and VP requests. It uses DID service endpoints and credential definitions (public keys) for encrypted communication. While handling VCs and VPs, the \textit{Aries Agent} calls the \textit{Indy Agent} to fetch/update credential schema and definitions, and revocation lists. The \textit{Controller}, implemented using \texttt{Node.js} orchestrates the identity initialization, exchange and validation flow as described in Section~\ref{subsec:messageflow}. It is responsible for fetching its associated MSP's latest root and intermediate certificates for sharing with foreign networks. These three modules run within a single Docker container. Lastly, an \textit{IIN Fabric Client} application built on the \texttt{Fabric SDK}~\cite{fabric-sdk} updates foreign networks' identities and certificates on the channel ledger using CMDAC transactions. This app, running within its own container, takes transaction requests from the \textit{Controller} and executes an application level signature collection flow (see Section~\ref{subsec:sig-flow}) before invoking the CMDAC.




\subsection{Protocol: Syncing Foreign Identities through Consensus} \label{subsec:sig-flow}

Our protocol implementation follows the steps described in Section~\ref{subsec:messageflow} verbatim except for the final step in which a foreign network's identities are recorded onto the local ledger. This step requires DLT-specific mechanisms, and we will show how it was implemented in Fabric. As an example, we consider the scenario where SWT is trying to fetch and sync the certificates of the Carrier organization in STL.
%In our implementation, the final step of identity configuration from the \textit{identity plane} to the \textit{data plane} is configuring the CMDAC with the Fabric certificates of an organization in the other network. Let us consider the example where Buyer organization is configuring the CMDAC of SWT with Carrier organization's fabric certificates. Here, the CMDAC can only be updated if the transaction for updation is validated and endorsed by others in SWT, namely, Seller, Buyer's bank and Seller's bank.

Recording the STL Carrier's certificates on the ledger creates a shared truth for the entire SWT network, enabling its peers to refer to those certificates in a data transfer session, either for access control or proof verification. Allowing the CMDAC to directly query IINs or foreign networks' agents to fetch these certificates would create a non-determinism hazard. Therefore, we use an application-level flow involving IIN Agents to obtain the information and submit a transaction to the CMDAC, which can then process the input in a deterministic manner.
%Hyperledger Fabric chaincode execution are supposed to be deterministic to ensure successful collection of endorsements with consistent read-write sets. Thus, the endorsement collection step during a chaincode transaction execution is only restricted to checks based on the ledger state, rather than any arbitrary operation like an API call over the network. As a result, the current Fabric implementation does not allow the organizations to query their respective \textit{IIN Agents} in the middle of a chaincode execution process. To circumvent this problem, we resort to collection of signatures in a separate application layer flow before submitting the CMDAC transaction as described next.

The SWT Buyer IIN Agent initiates this flow by validating the STL Carrier's Membership VC with the IIN, and subsequently fetches the Carrier's certificates from the  Carrier's IIN Agent (whose service endpoint is part of the Carrier's DID record). The Buyer IIN Agent then sends these certificates to its Fabric Client app, which then prepares a \textit{signature collection request}, and sends it to the Fabric Client of the SWT Seller IIN Fabric Client app. The latter validates the Carrier's certificates after consultation with their own IIN Agents (who have presumably fetched those certificates too), and then counter-signs the request on behalf of its organization. The Buyer aggregates the responses (only one here) and submits it as input in a CMDAC transaction. The chaincode checks for the presence of valid signatures from every SWT organization (here: Buyer and Seller) before approving the update of the STL Carrier's identity state on the ledger. Note that this update is idempotent, and can be carried out concurrently by the IIN Agents of both Buyer and Seller. Also, if the Buyer's and Seller's IIN Agents' copies of Carrier certificates are not in sync, the signature collection flow will fail and must be retried.
%Considering the example above, the IIN Agent of the Buyer organization validates the SSI and Membership VC of Carrier in the \textit{identity plane} and then fetches the Fabric root and intermediate certificate which needs to be configured in CMDAC. Buyer IIN Agent sends the CMDAC update request to the Fabric Client application, which then prepares a \textit{signature collection request}, and sends it to the Fabric Client of Seller, Buyer's bank and Seller's bank. Each of those Fabric Clients upon receipt of the signature collection requests validates the Carrier's Fabric certificates in consultation with their own IIN Agents, and finally returns the signed response.
%The Buyer Fabric Client aggregates all the signatures and submits it as a transaction to the CMDAC chaincode. The chaincode validation logic checks for the signatures in the transaction and updates the Carrier's Fabric certificates in the ledger. This application layer flow ensures that even if certain organization's IIN Agent is not in sync with the others in terms of fetching the up-to-date identity information, the identity updation process will fail gracefully in the application level, which can be retried. While, the chaincode execution process remains deterministic.

This protocol replaces the naive implementation in Abebe et al~\cite{abebe2019enabling} where organizational identities and root and intermediate certificates were fetched out-of-band manually and recorded on the local ledgers during bootstrap. The identity plane exchange we have demonstrated makes the process more secure and consensus-based. Further, any changes in organizational memberships or certificate belonging to an organizations can be determined and synced automatically through periodic queries made to the IIN registry (for membership and revocation lists) or whenever a proof validation fails because of expired certificates.

\subsection{Identity Network and Trust Anchors}

We deployed a single IIN, an Indy network bootstrapped with 4 independent Sovrin stewards~\cite{sovrin}. Two trust anchors were enrolled in the IIN by the stewards: one in the name of IBM to represent the SWT consortium and another in the name of Maersk to represent STL (see Figure~\ref{fig:trade-flow-implementation}). (Note that IBM and Maersk are initiators and major players in the real We.Trade and TradeLens networks respectively, and are therefore realistic sources of trust.) A single IIN with two trust anchors is sufficient to demonstrate operational mechanics in a proof-of-concept; in a production implementation, we will likely have more diversity but the mechanisms used will be identical to what we demonstrate here. The SWT Seller and Buyer register verinyms with, and obtain Membership VCs from, the IBM anchor in the IIN; likewise, the STL Seller and Carrier register and obtain theirs from the Maersk anchor.
%In our proof-of-concept implementation with SWT and STL, we construct the IIN with \textit{IIN Agents} of all the organizations of the two networks, and two trust anchors: IBM, and Maersk. The Indy network is bootstrapped with 4 independent Stewards, who then enroll IBM and Maersk as TRUSTEES. IBM is the organization involved in deploying  SWT network, and is thus a well known organization that can be considered a DID validator as well as Membership validator for SWT. Similarly, Maersk is the most well known stakeholder of TradeLens, and therefore functions as the trust anchor for validating STL. We use only two trust anchors for the sake of the simple proof-of-concept implementation, and in real world scenarios there can be multiple trust anchors in different combinations as discussed in Sec \ref{}. Seller, Buyer,  and  the  Seller’s  and  Buyer’s  banks register their \textit{Verinym} and obtain their Membership VC for SWT from IBM trust anchor. On the other hand Carrier obtains its Verinym and Membership VC from Maersk. The Seller organization that is member of both SWT and STL also  obtains the Membership VC for SWT from Maersk.
%The \textit{IIN Agents} seamlessly automate the entire process of SSI exchange and validation, obtaining blockchain specific certificates, and finally configuring them in CMDAC chaincode. This eliminates the manual pre-configuration step for identities as in Abebe et al \cite{abebe2019enabling}, and allows the two different blockchain networks to carry out verifiable data transfer. In case any blockchain credentials are updated and the data acceptance validation phase fails in CMDAC, it triggers an update in the IIN Agents to fetch the new Fabric certificates. Moreover, the IIN Agents periodically check the revocation registry accumulators in Indy, and also the Memberlist VPs, to detect changes in the membership structure of the networks.
